Robust End-to-End Focal Liver Lesion Detection using Unregistered Multiphase Computed Tomography Images

The computer-aided diagnosis of focal liver lesions (FLLs) can help improve workflow and enable correct diagnoses; FLL detection is the first step in such a computer-aided diagnosis. Despite the recent success of deep-learning-based approaches in detecting FLLs, current methods are not sufficiently robust for assessing misaligned multiphase data. By introducing an attention-guided multiphase alignment in feature space, this study presents a fully automated, end-to-end learning framework for detecting FLLs from multiphase computed tomography (CT) images. Our method is robust to misaligned multiphase images owing to its complete learning-based approach, which reduces the sensitivity of the model's performance to the quality of registration and enables a standalone deployment of the model in clinical practice. Evaluation on a large-scale dataset with 280 patients confirmed that our method outperformed previous state-of-the-art methods and significantly reduced the performance degradation for detecting FLLs using misaligned multiphase CT images. The robustness of the proposed method can enhance the clinical adoption of the deep-learning-based computer-aided detection system.

==> 6.Discussion.tex <==
\section{Discussion}
To perform a fair and unbiased model evaluation without data leakage, the custom dataset is split prior to the experiment without any manual data examination. Consequently, the values of the test set metrics were higher than those of the validation set metrics across all the experiments (IoU50 and IoBB50 in Table \ref{ap_result} and \ref{ablation}). This was due to the 10 patients in the test set who had HCC sizes that were larger than the average size, which facilitated detection by all the model configurations. However, this is not a concerning factor as the test set metrics were consistent for all the models, and the relative scale was maintained throughout the configurations, indicating that none of the models had overfitted to the training set.

This study demonstrated a significantly improved detection performance by applying the proposed methods to two fundamentally different approaches for object detection, namely the GSSD \cite{lee2018liver} and PixelLink \cite{deng2018pixellink}; this implies that the proposed method is transferable to various single-stage detection models. Based on the performance evaluation results with various metrics (Table \ref{figure_compare}), PixelLink++ performed significantly better than other methods (including GSSD++) on the validation set, with a less stringent overlap threshold. PixelLink \cite{deng2018pixellink} cast the bounding box regression problem into instance segmentation and used balanced cross-entropy loss for a small area, enabling PixelLink-based models to excel at detecting smaller-sized lesions from the validation set. However, owing to the noisy post-filtering approach for the bounding box extraction from the predicted segmentation map, the performance degraded for metrics with a higher overlap threshold. SSD \cite{liu2016ssd} and RetinaNet \cite{lin2017focal} used a more conventional approach involving the use of a predefined set of densely distributed anchor boxes \cite{ren2015faster}, and achieved better performances on metrics with higher thresholds.
